Approximate Matrix Multiplication with Application to Linear Embeddings

In this paper, we study the problem of approximately computing the product of two real matrices. In particular, we analyze a dimensionality-reduction-based approximation algorithm due to Sarlos [1], introducing the notion of nuclear rank as the ratio of the nuclear norm over the spectral norm. The presented bound has improved dependence with respect to the approximation error (as compared to previous approaches), whereas the subspace -- on which we project the input matrices -- has dimensions proportional to the maximum of their nuclear rank and it is independent of the input dimensions. In addition, we provide an application of this result to linear low-dimensional embeddings. Namely, we show that any Euclidean point-set with bounded nuclear rank is amenable to projection onto number of dimensions that is independent of the input dimensionality, while achieving additive error guarantees.

==> contributions.tex <==
\section{Our Contributions}
Here, we highlight the main contributions of this manuscript:
\begin{enumerate}
\item [$(i)$] We provide a novel analysis on the approximate matrix multiplication problem based on the notion of nuclear rank (See Theorem~\ref{thm:main}).
\item [$(ii)$] We demonstrate an application of the approximate matrix multiplication bound to dimensionality reduction with relative guarantees. %, i.e., reduction of a dataset to dimensions that depend on its intrinsic dimensionality (in contrast to the logarithmic dependency on the number of points as in the JL lemma~\cite{johnson1984extensions}).
\end{enumerate}
To highlight the potential of the second contribution, consider the scenario of an almost one-dimensional point set, i.e., randomly generated points centred around a line with small variance in high dimensional space. In this setting, intuitively we expect that a constant number of dimensions are necessary in order to preserve the geometry of the dataset. However, the JL lemma~\cite{johnson1984extensions} (pessimistically) proposes that logarithmic number of dimensions is necessary, which contradicts out expectations for less dimensions.


%As an illustrative example for the second contribution, consider the following scenario of a point-set that is almost one dimensional, i.e., randomly generated points around a linear in high dimensional space. In this setting, we expect that constant number of dimensions are necessary in order to preserve the geometry of this point-set. However, the JL lemma (pessimistically) proposes that logarithmic number of dimensions are necessary.****

==> experiments.tex <==
\section{Experiments}
